MultiTalk: A Highly-Branching Dialog Testbed for Diverse Conversations

We study conversational dialog in which there are many possible responses to a given history. We present the MultiTalk Dataset, a corpus of over 320,000 sentences of written conversational dialog that balances a high branching factor (10) with several conversation turns (6) through selective branch continuation. We make multiple contributions to study dialog generation in the highly branching setting. In order to evaluate a diverse set of generations, we propose a simple scoring algorithm, based on bipartite graph matching, to optimally incorporate a set of diverse references. We study multiple language generation tasks at different levels of predictive conversation depth, using textual attributes induced automatically from pretrained classifiers. Our culminating task is a challenging theory of mind problem, a controllable generation task which requires reasoning about the expected reaction of the listener.

==> fig/task0_graph.tex <==
\begin{figure}[t]

\begin{center}
\includegraphics[width=0.99\linewidth]{fig/realtalk_figure_task0.pdf}
\end{center}

\caption{
    TODO
}
\label{fig:task0_graph}
\end{figure}

==> fig/task1_human_eval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}
{\begin{tabular}{@{}llccc@{}}
\toprule
\textbf{Model} & \textbf{Setup} & \textbf{Emotion Correctness} & \multicolumn{1}{p{3cm}}{\centering \textbf{Relevance}}  & \multicolumn{1}{p{3cm}}{\centering \textbf{Fluency} } \\ \midrule
GPT-2 M & & 1.59 &  2.01   &  2.34 \\
Dialog Tree Model & & 1.64  &  \textbf{2.35}  &    \textbf{2.63}  \\
Retrieval & most likely &  1.63   &  2.00   &    2.54 \\
 & w/ emotion $e$ &  2.13   &  1.85   &    2.56 \\ 
Emotion-Aware Model  & normal  &    \textbf{2.18}    &  2.26 &   2.57 \\
 & oversampled  &   2.11   &  2.11 &   2.55 \\
\bottomrule
\end{tabular}}
\caption{
\textcolor{red}{The Human Evaluation task performance for the Emotion-Conditioned Generation.}
%Finetuned GPT-2 Medium achieves lowest perplexity (PPL), and also gets the best scores on both Matching Metric (BLEU-4) and Matching Metric (ROUGE-L f1).
}
\label{tab:task1_human_eval}
\end{table}

==> src/results.tex <==
% \section{Quantitative Results}
% We show the effectiveness of the Matching metric in task 0,and evaluate all models based on their ability to generate response with given prompt, history and emotion in task 1 or lookahead emotion in task 2.
% \subsection{Automatic Metrics}
% In task 0, as we mention in the Experiments section, we calculate Matching metric (BLEU-4), Matching metric (ROUGE-L f1) and perplexity. In task 1 and task 2, we compute perplexity and emotion accuracy for all models to measure the quality of their generations, where perplexity is computed by the finetuned GPT2 model and emotion accuracy is the number of generations with correct labeled emotion divided by the total number of generations. To be more specific, emotion accuracy in task 1 is calculated based on generations $R1$ and emotion accuracy in task 2 is calculated based on children generations $R2$.

% \subsection{Task 0}
% \input{fig/task0_table}
% Dialog Tree Model achieves the lowest perplexity, which also improves a lot compared with the best pretrained model GPT-2 XL. 
% All of five models get low score on Matching Metric (BLEU-4), which shows that they all generate very different sentences from 10 gold references.
% However, with leading on both Matching Metric (BLEU-4) and Matching Metric (ROUGE-L), Dialog Tree Model is more likely to generate diverse and good quality sentences.

\subsection{Task 1}
\input{fig/task1}
\subsubsection*{Pretrained GPT-2 Medium}
From Table~\ref{tab:task1}, Pretrained GPT-2 Medium gets the highest perplexity and lowest Average emotion accuracy among all models. 

\subsubsection*{Dialog Tree Model}
Dialog Tree Model gets the lowest perplexity but a very low emotion accuracy.

\subsubsection*{Retrieval Model}
Using the retrieval most likely setup, the perplexity is lower than using the retrieval with emotion E setup. Because retrieval with emotion E always retrieve a generation with emotion E from training set, so the emotion accuracy is 1. 

\subsubsection*{\emoModelName~}
\emoModelName~in both setup achieves much better emotion accuracy and low perplexity comparing with other models. 
Oversampled setup improves the emotion accuracy about $2$ percent from $0.513$ to $0.536$ with a little bit trade off on perplexity comparing with the normal setup.

\subsection{Task 2}
\input{fig/task2}
\subsubsection*{Pretrained GPT-2 Medium}
Pretrained GPT-2 Medium achieves poor perplexity and emotion accuracy at Task 2, which is expected.  

\subsubsection*{Dialog Tree Model}
Dialog Tree Model achieves good perplexity and a decent emotion accuracy.
\subsubsection*{Retrieval Model}
From Table~\ref{tab:task2}, retrieval with emotion E has better average emotion accuracy but a little bit worse perplexity than the other two Retrieval model setups. And its emotion accuracy is highest among all the models.

\subsubsection*{\emoModelName~}
Similar to the retrieval model performance, the Emotion model conditioned on emotion E has better emotion accuracy than the Emotion model conditioned on $T[\rightarrow E]$. 

\subsubsection*{Lookahead Model}
Although both Lookahead Model setups gets lower emotion accuracy than Retrieval model and Emotion-Aware Model, they have relatively low perplexity.
Especially, the Lookahead Model with normal setup gets the lowest perplexity among all models. 


\section{Qualitative Results}

\subsection{\emoModelName~}
\paragraph{Positive Findings}
From the first two examples, (a) and (b), in Figure \ref{fig:lookahead_examples}, we can see \emoModelName~is able to generate high-quality sentence and with given emotion. 
More interestingly, the first example, (a), shows that \emoModelName~is able to turn the vibe of the conversation into an opposite direction quickly but in a reasonable way. 
More specifically, the whole vibe for the previous conversation is joy. 
Now, given a sadness emotion, the model generates this high quality sentence which not only relates to the previous context but also contains sadness emotion.
\paragraph{Error Analysis}
The third example, (c), in Figure \ref{fig:lookahead_examples} shows a weakness of Emotion-Aware Model. 
Although Emotion-Aware Model can always generate sentences with given emotion, sometimes the context of generation doesn't make sense in current situation and may controvert the meaning of previous conversation.

\input{fig/lookahead_figure}

\subsection{\modelName~}
\paragraph{Positive Findings} 
Both first two examples, (d) and (e), in Figure \ref{fig:lookahead_examples} shows that \modelName~sometimes can generate high-quality sentence that leads to future responses with given emotion, and it learns to generate affirmative sentence to lead a potential positive response and generate negative sentence in order to lead a potential negative response. 

\paragraph{Error Analysis} 
In the leading emotion perspective, the third example, (f), in Figure \ref{fig:lookahead_examples} looks good because the generation for Mildred can lead to a angry response from Keith although the response for Keith is with surprise emotion.
However, it is bad at relevance and realistic perspective: the generation doesn't relate much to previous conversation, and it is unrealistic.



